A hybrid reduced-order model for segregated fluid-structure interaction solvers in an ALE approach at high Reynolds number

This study introduces a first step for constructing a hybrid reduced-order models (ROMs) for segregated fluid-structure interaction in an Arbitrary Lagrangian-Eulerian (ALE) approach at a high Reynolds number using the Finite Volume Method (FVM). The ROM is driven by proper orthogonal decomposition (POD) with hybrid techniques that combines the classical Galerkin projection and two data-driven methods (radial basis networks , and neural networks/ long short term memory). Results demonstrate the ROM ability to accurately capture the physics of fluid-structure interaction phenomena. This approach is validated through a case study focusing on flow-induced vibration (FIV) of a pitch-plunge airfoil at a high Reynolds number 10000000.

==> sections/discussion.tex <==
The first part discusses the sensitivity of the number of basis functions to the accuracy of the solution for the Galerkin projection. Then, a comment on the reconstruction of structural displacements is made. 
Lastly, we argue about the model and the results obtained using RNNs/NNs.
\subsubsection{Sensitivity study on number of basis vectors} 
In this study, the relative $L^2$ errors for velocities, pressure, and apparent viscosity are compared to provide a quantitative measurement of both model's (FOM and ROM) performance. The relative $L^2$ error is computed as:
\begin{eqnarray}\label{RelError}
    \epsilon_u = \displaystyle\frac{||\boldsymbol{u}_{FOM} -\boldsymbol{u}_{ROM} ||_{L^2(\Omega)}}{||\boldsymbol{u}_{FOM}||_{L^2(\Omega)}}\times 100\% ~~~ \epsilon_p = \displaystyle\frac{||p_{FOM} - p_{ROM} ||_{L^2(\Omega)}}{||p_{FOM}||_{L^2(\Omega)}}\times 100\%
\end{eqnarray}
As illustrated in \cref{fig:errorsfields} the Galerkin projection achieves greater accuracy when more POD modes are used for reconstruction. In this illustration, it is seen that with $N_u = N_p = 10$ the error velocity lies between 0-0.05 \%  mostly. In practice, it is important to ensure that the number of modes used is not too large as this can require more time's reconstruction/ prediction to be more expensive compared to the full-order time as one can see in \cref{tab:OffOnline}. \textit{Additionally, the matrix multiplication every time step is also computationally expensive in the online phase as the algorithm still has a dependency on the original number of degrees of freedom}. To judge how well the reduced-order model fits the full-order model, an analysis at the local level is done. This analysis compares the forces reconstruction in \cref{fig:forces} for both models, varying the number of modes of the velocities and pressure.
\subsubsection{Structural displacement via POD-RBF}
The results indicate that the energy is concentrated in the first 3 POD modes for the pointDisplacement field as shown in \cref{fig:eigdecay} and \cref{tab:eigenvectors}.
This observation implies that the ALE field can be reduced with just three POD modes instead of 26 316 grid nodes.
As such, it can be seen from \cref{fig:AirfoilMotion} that the radial basis network used to reconstruct the structural motion solution has quite good agreement with the high-fidelity solution during the time window. It can be also seen that the amplitudes and frequencies match pretty well.
And the accuracy depends on the POD basis of the velocity, and pressure this is due to the presence of the lift forces in the \cref{structmotion1,structmotion2} and these forces are computed using the velocity and the pressure.
\subsubsection{Neural Network Training }
Having verified the efficacy of the present approach for the velocity, pressure, and point displacement in the above subsections,  this part turns the attention to ML predictions. To assess if the field reconstruction of the eddy viscosity from the neural network is accurate, the truth temporal coefficients of the POD decomposition and the predicted ones coming from the feed-forward neural network can be directly compared as one can see in \cref{fig:nutCoeffs}. 
%From (table....), the neural network architecture can be visualized. 
For all the training runs in this work, a variant of the stochastic gradient descent algorithm called adaptive moment estimation ADAM \cite{kingma2017adam} is used. ADAM has an adaptive learning rate method which is commonly used to train deep networks. The evolution of each  scaled temporal mode is given by:
\begin{equation}
    \hat{\boldsymbol{a}}_j(t) = \frac{\boldsymbol{a}_j(t) - \left<\boldsymbol{a}_j(t)\right>}{\sigma[\boldsymbol{a}_j(t)]}
\end{equation}
A scaling of the dataset is necessary to have correct training of the network, otherwise, the gradients that enter the computations of the cost function will be too small and it will be impossible to generate significant updates of the parameters of the network \cite{borrelli2022predicting}. The model parameters  (weights and bias) are trained with the PyTorch library  \cite{paszke2019pytorch} and later exported in the C++ area to generate the transient predicted solution at the online level.
% \begin{figure}[H]
% \centering
% \includegraphics[width=0.5\textwidth]{images/feedforwardnns.png}
% \caption{Schematic view of a fully connected NN composed of three layers: input, hidden layer, and output layer.}
% \label{fig:feednns}
% \end{figure}
The main building blocks of the feed-forward NNs contain six layers:  an input layer which is the vector of temporal coefficients of the velocity, four hidden layers of size 64 followed by a LeakyReLU activation function,  and the output layer which is the temporal coefficients of the eddy viscosity. 
%\cref{fig:feednns} gives a visualization of the model.
The training is conducted on a random sample of both temporal coefficients of velocity and eddy viscosity. 80\% of the data are used for training and the remaining for validation. 
%\textbf{The training and validation errors for the feed-forward neural network are plotted in......}. \textbf{Then, the model parameters (weights and bias) are trained with the PyTorch library \cite{paszke2019pytorch} and later exported in a C++ environment to generate the transient predicted solution at the online level.}

For LSTM-RNNs, an LSTM encoder-decoder model is used for training and validation on the data set as illustrated in \cref{fig:lstm-encdec}. The model can capture the trend of the reference data both on the train and validation data. The architecture of the LSTM-Encoder-Decoder model has one LSTM layer in the encoder part and another LSTM layer in addition to one hidden layer of 5 neurons in the decoder part. The reason for the choice is that this model has been used extensively for sequence-to-sequence prediction in the literature for NLP (natural language processing). 
%In \cref{fig:LstmCoeffs}, one can see that the trend of the predicting coefficients behaves as a purely random walk.  
In \cref{fig:LstmCoeffs}, one can observe that the phase portrait of the predicting coefficients using LSTM can reproduce the initial phase portrait with too much oscillation. Even though the frequencies of both signals are different, the predicted amplitudes belong to the range of the reference amplitudes. With the periodic trend of the predicted coefficients, it can be inferred that the Lyapunov exponent defined in \cref{LyapoExpo} is negative. Furthermore, the accuracy of the predicting coefficients may also be theoretically restricted due to the Lyapunov exponent theory for dynamical systems \cite{sprott2003chaos}. The Lyapunov exponent tells us that the farther in time we move from the initial state $\boldsymbol{x}_0$, the greater the rate of divergence between trajectories that were closer as $t \rightarrow 0$. Intuitively, in a dynamical
system, the likelihood of making accurate predictions for time series farther away from the origin, drops exponentially as proposed by \cite{mohan2018deep}. Hence, this merely indicates that the accurate, pure data-driven approaches to the prediction of long-time horizons may have several difficulties.
\begin{align}\label{LyapoExpo}
  \|\delta \boldsymbol{A}(t)\| \approx e^{\lambda t}\|\delta \boldsymbol{A}_0\|.  
\end{align}
%Simulations show that increasing the number of neurons in the training/validation improves the results. 
It is observed at the online level an oscillation phenomenon which was also observed in \cite{borrelli2022predicting} in the prediction of the velocity field in the channel flow. In their study, they reported that the phenomenon was due to an insufficient number of snapshots of the training dataset or when the number of cells in the hidden layer was not enough. Together with that, one can add sensitivity to the initial condition as one can observe in \cref{fig:LstmCoeffs}. It is also possible that the memory in the sequence can affect the LSTM accuracy as reported in \cite{mohan2018deep} because signals originating from chaotic dynamic systems are known to have quite short correlated events and memory does not typically persist over long periods. In this case, the Hurst exponent is a prominent solution \cite{hurst1951long} for further investigations. However, the mentioned suggestions were not the emphasis of this paper. Instead, the emphasis was concentrated on the design of the overall algorithm to generate a reduced-order model for segregated FSI solvers in the FV context.
% - \textbf{More data for the testing to achieve more accuracy.}
% - \textbf{Over fitting} issue
% - While LSTM was more accurate, it was seen that its accuracy deteriorated with an increase in horizon 
% \textbf{In order to further analyze the quality of the predictions, we assessed whether the dynamic behavior of the predicted flow was consistent with the reference model.}
% \textbf{The reason for this discrepancy lies in the nature of the nine-equation model, which is a
% dynamical system in which very small perturbations lead to a completely different temporal evolution of the modes.}
% -\textbf{By reducing the number of POD coefficients, it is shown that we have to reduce the hidden size and the number of epochs of training.}
%- Quantify memory using Hurst exponent.
